Towards Novel Target Discovery Through Open-Set Domain Adaptation

Open-set domain adaptation (OSDA) considers that the target domain contains samples from novel categories unobserved in external source domain. Unfortunately, existing OSDA methods always ignore the demand for the information of unseen categories and simply recognize them as "unknown" set without further explanation. This motivates us to understand the unknown categories more specifically by exploring the underlying structures and recovering their interpretable semantic attributes. In this paper, we propose a novel framework to accurately identify the seen categories in target domain, and effectively recover the semantic attributes for unseen categories. Specifically, structure preserving partial alignment is developed to recognize the seen categories through domain-invariant feature learning. Attribute propagation over visual graph is designed to smoothly transit attributes from seen to unseen categories via visual-semantic mapping. Moreover, two new cross-main benchmarks are constructed to evaluate the proposed framework in the novel and practical challenge. Experimental results on open-set recognition and semantic recovery demonstrate the superiority of the proposed method over other compared baselines.

==> I2AwA_open.tex <==

\begin{table}[t]
\caption{Open-set domain adaptation Accuracy ($\%$) on \textit{I2AwA}} 
\label{table:I2AwA_open}
\linespread{1.3} 
\centering
\scriptsize
\setlength{\tabcolsep}{6pt} % Default value: 6pt 
\renewcommand{\arraystretch}{1} % Default value: 1 
\begin{tabular}{cccc}

\toprule
% & \multicolumn{2}{c}{\textbf{I2AwA}}\\
% % \cmidrule(lr){2-3}
% \hline
Method & OS$^*$  & OS$^\diamond$ & OS\\
\hline
OSBP \cite{saito2018open} & 67.63 & 7.54 & 66.16\\

STA \cite{liu2019separate} & 51.52 & 45.5 & 51.37 \\

AOD \cite{feng2019attract} & 75.21 & 6.31 & 73.53 \\


\hline
Ours(Init) & 82.20 & 65. 28 & 81.79 \\

Ours(Vis) & 48.16 & 70.33 & 48.70 \\

Ours  & 83.15 & 70.20 & 82.83 \\
\bottomrule
\end{tabular}\vspace{-6mm}

\end{table}


==> I2AwA_semantic.tex <==

\begin{table}[t]
\caption{Semantic Recovery Accuracy ($\%$) on I2AwA} 
\label{table:I2AwA_semantic}
\linespread{1.3} 
\centering
\setlength{\tabcolsep}{6pt} % Default value: 6pt 
\renewcommand{\arraystretch}{1} % Default value: 1 
\begin{tabular}{cccc}

\toprule
% & \multicolumn{2}{c}{\textbf{I2AwA}}\\
% % \cmidrule(lr){2-3}
% \hline
Method & S  &  U & H\\
\hline







Source-only & 77.22 & 0.34 & 0.68\\

ABP \cite{zhu2019learning} & 79.79 & 0.00 & 0.00 \\


TF-VAE \cite{narayan2020latent}
& 62.83 & 0.00 & 0.00\\

\hline
ABP* \cite{zhu2019learning} & 77.99 & 13.42 & 22.90\\
TF-VAE* \cite{narayan2020latent}
& 37.74 & 20.04 & 26.18\\

\hline

Ours  & 83.08 & 22.02 & 34.81 \\
\bottomrule
\end{tabular}

\end{table}


==> ablation.tex <==

\begin{table}[t]
\caption{Open-Set Accuracy ($\%$) on I2AwA} 
\label{table:ablation}
\linespread{1.3} 
\centering
\setlength{\tabcolsep}{3pt} % Default value: 6pt 
\renewcommand{\arraystretch}{1} % Default value: 1 
\begin{tabular}{ccccccc}

\toprule
Task & \multicolumn{3}{c}{\textbf{Open-set}} & \multicolumn{3}{c}{\textbf{Semantic Recovery}}\\

\cmidrule(lr){2-4}
\cmidrule(lr){5-7}

Method & OS$^*$ & OS$^\diamond$ & OS & S & U & H \\
\hline
W/o R & 78.22 & 70.83 & 78.04 & 80.79 & 20.24 & 32.37 \\ %$\mathcal{L}^R$ 
W/o D & 75.6 & 73.81 & 75.56 & 77.41 & 16.35 & 27.00 \\
W/o AP & 82.56 & 70.43 & 82.26 & 82.81 & 18.30 & 29.98 \\
% 67.45 & 77.83 & 67.70 & 78.18 & 15.98 & 26.54 \\
W/o VS & 70.54 & 70.1 & 70.53 & 84.83 & 12.72 & 22.12 \\
\hline
Ours  & 83.15 & 70.20 & 82.83 & 83.08 & 22.02 & 34.81  \\
\bottomrule
\end{tabular}

\end{table}


==> bib_error.tex <==
%  @inproceedings{rodriguez2020embedding,
%   title={Embedding propagation: Smoother manifold for few-shot classification},
%   author={Rodr{\'\i}guez, Pau and Laradji, Issam and Drouin, Alexandre and Lacoste, Alexandre},
%   booktitle={European Conference on Computer Vision},
%   pages={121--138},
%   year={2020},
%   organization={Springer}
% }
@inproceedings{rodriguez2020embedding,
  title={Embedding propagation: Smoother manifold for few-shot classification},
  author={Rodr{\'\i}guez, Pau and Laradji, Issam and Drouin, Alexandre and Lacoste, Alexandre},
  booktitle={European Conference on Computer Vision},
  pages={121--138},
  year={2020},
  organization={Springer}
}

% @inproceedings{he2016deep,
%   title={Deep residual learning for image recognition},
%   author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
%   booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
%   pages={770--778},
%   year={2016}
% }

@inproceedings{he2016deep,
  title={Deep residual learning for image recognition},
  author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={770--778},
  year={2016}
}

% @inproceedings{huynh2020shared,
%   title={A shared multi-attention framework for multi-label zero-shot learning},
%   author={Huynh, Dat and Elhamifar, Ehsan},
%   booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
%   pages={8776--8786},
%   year={2020}
% }

@inproceedings{huynh2020shared,
  title={A shared multi-attention framework for multi-label zero-shot learning},
  author={Huynh, Dat and Elhamifar, Ehsan},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8776--8786},
  year={2020}
}

% @inproceedings{snell2017prototypical,
%   title={Prototypical networks for few-shot learning},
%   author={Snell, Jake and Swersky, Kevin and Zemel, Richard},
%   booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
%   pages={4080--4090},
%   year={2017}
% }

@inproceedings{snell2017prototypical,
  title={Prototypical networks for few-shot learning},
  author={Snell, Jake and Swersky, Kevin and Zemel, Richard},
  booktitle={Proceedings of the 31st International Conference on Neural Information Processing Systems},
  pages={4080--4090},
  year={2017}
}

% @article{zhou2004learning,
%   title={Learning with local and global consistency},
%   author={Zhou, Dengyong and Bousquet, Olivier and Lal, Thomas Navin and Weston, Jason and Sch{\"o}lkopf, Bernhard},
%   journal={Advances in neural information processing systems},
%   volume={16},
%   number={16},
%   pages={321--328},
%   year={2004}
% }

@article{zhou2004learning,
  title={Learning with local and global consistency},
  author={Zhou, Dengyong and Bousquet, Olivier and Lal, Thomas Navin and Weston, Jason and Sch{\"o}lkopf, Bernhard},
  journal={Advances in neural information processing systems},
  volume={16},
  number={16},
  pages={321--328},
  year={2004}
}

% @inproceedings{dong2020cscl,
%   title={CSCL: Critical Semantic-Consistent Learning for Unsupervised Domain Adaptation},
%   author={Dong, Jiahua and Cong, Yang and Sun, Gan and Liu, Yuyang and Xu, Xiaowei},
%   booktitle={European Conference on Computer Vision},
%   pages={745--762},
%   year={2020},
%   organization={Springer}
% }
@inproceedings{dong2020cscl,
  title={CSCL: Critical Semantic-Consistent Learning for Unsupervised Domain Adaptation},
  author={Dong, Jiahua and Cong, Yang and Sun, Gan and Liu, Yuyang and Xu, Xiaowei},
  booktitle={European Conference on Computer Vision},
  pages={745--762},
  year={2020},
  organization={Springer}
}

% @article{long2017conditional,
%   title={Conditional adversarial domain adaptation},
%   author={Long, Mingsheng and Cao, Zhangjie and Wang, Jianmin and Jordan, Michael I},
%   journal={arXiv preprint arXiv:1705.10667},
%   year={2017}
% }

@article{long2017conditional,
  title={Conditional adversarial domain adaptation},
  author={Long, Mingsheng and Cao, Zhangjie and Wang, Jianmin and Jordan, Michael I},
  journal={arXiv preprint arXiv:1705.10667},
  year={2017}
}


% @inproceedings{pan2020exploring,
%   title={Exploring category-agnostic clusters for open-set domain adaptation},
%   author={Pan, Yingwei and Yao, Ting and Li, Yehao and Ngo, Chong-Wah and Mei, Tao},
%   booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
%   pages={13867--13875},
%   year={2020}
% }
@inproceedings{pan2020exploring,
  title={Exploring category-agnostic clusters for open-set domain adaptation},
  author={Pan, Yingwei and Yao, Ting and Li, Yehao and Ngo, Chong-Wah and Mei, Tao},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={13867--13875},
  year={2020}
}

% @inproceedings{zhuo2019unsupervised,
%   title={Unsupervised open domain recognition by semantic discrepancy minimization},
%   author={Zhuo, Junbao and Wang, Shuhui and Cui, Shuhao and Huang, Qingming},
%   booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
%   pages={750--759},
%   year={2019}
% }

@inproceedings{zhuo2019unsupervised,
  title={Unsupervised open domain recognition by semantic discrepancy minimization},
  author={Zhuo, Junbao and Wang, Shuhui and Cui, Shuhao and Huang, Qingming},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={750--759},
  year={2019}
}

% @inproceedings{xian2017zero,
%   title={Zero-shot learning-the good, the bad and the ugly},
%   author={Xian, Yongqin and Schiele, Bernt and Akata, Zeynep},
%   booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
%   pages={4582--4591},
%   year={2017}
% }

@inproceedings{xian2017zero,
  title={Zero-shot learning-the good, the bad and the ugly},
  author={Xian, Yongqin and Schiele, Bernt and Akata, Zeynep},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={4582--4591},
  year={2017}
}

% @inproceedings{peng2019moment,
%   title={Moment matching for multi-source domain adaptation},
%   author={Peng, Xingchao and Bai, Qinxun and Xia, Xide and Huang, Zijun and Saenko, Kate and Wang, Bo},
%   booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
%   pages={1406--1415},
%   year={2019}
% }

@inproceedings{peng2019moment,
  title={Moment matching for multi-source domain adaptation},
  author={Peng, Xingchao and Bai, Qinxun and Xia, Xide and Huang, Zijun and Saenko, Kate and Wang, Bo},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={1406--1415},
  year={2019}
}

% @inproceedings{panareda2017open,
%   title={Open set domain adaptation},
%   author={Panareda Busto, Pau and Gall, Juergen},
%   booktitle={Proceedings of the IEEE International Conference on Computer Vision},
%   pages={754--763},
%   year={2017}
% }

@inproceedings{panareda2017open,
  title={Open set domain adaptation},
  author={Panareda Busto, Pau and Gall, Juergen},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={754--763},
  year={2017}
}

% @inproceedings{deng2009imagenet,
%   title={Imagenet: A large-scale hierarchical image database},
%   author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
%   booktitle={2009 IEEE conference on computer vision and pattern recognition},
%   pages={248--255},
%   year={2009},
%   organization={Ieee}
% }

@inproceedings{deng2009imagenet,
  title={Imagenet: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={2009 IEEE conference on computer vision and pattern recognition},
  pages={248--255},
  year={2009},
  organization={Ieee}
}


% @inproceedings{kundu2020towards,
%   title={Towards inheritable models for open-set domain adaptation},
%   author={Kundu, Jogendra Nath and Venkat, Naveen and Revanur, Ambareesh and Babu, R Venkatesh and others},
%   booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
%   pages={12376--12385},
%   year={2020}
% }

@inproceedings{kundu2020towards,
  title={Towards inheritable models for open-set domain adaptation},
  author={Kundu, Jogendra Nath and Venkat, Naveen and Revanur, Ambareesh and Babu, R Venkatesh and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12376--12385},
  year={2020}
}

% @inproceedings{feng2019attract,
%   title={Attract or distract: Exploit the margin of open set},
%   author={Feng, Qianyu and Kang, Guoliang and Fan, Hehe and Yang, Yi},
%   booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
%   pages={7990--7999},
%   year={2019}
% }
@inproceedings{feng2019attract,
  title={Attract or distract: Exploit the margin of open set},
  author={Feng, Qianyu and Kang, Guoliang and Fan, Hehe and Yang, Yi},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={7990--7999},
  year={2019}
}

% @inproceedings{liu2019separate,
%   title={Separate to adapt: Open set domain adaptation via progressive separation},
%   author={Liu, Hong and Cao, Zhangjie and Long, Mingsheng and Wang, Jianmin and Yang, Qiang},
%   booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
%   pages={2927--2936},
%   year={2019}
% }

@inproceedings{liu2019separate,
  title={Separate to adapt: Open set domain adaptation via progressive separation},
  author={Liu, Hong and Cao, Zhangjie and Long, Mingsheng and Wang, Jianmin and Yang, Qiang},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={2927--2936},
  year={2019}
}

% @inproceedings{saito2018open,
%   title={Open set domain adaptation by backpropagation},
%   author={Saito, Kuniaki and Yamamoto, Shohei and Ushiku, Yoshitaka and Harada, Tatsuya},
%   booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
%   pages={153--168},
%   year={2018}
% }

@inproceedings{saito2018open,
  title={Open set domain adaptation by backpropagation},
  author={Saito, Kuniaki and Yamamoto, Shohei and Ushiku, Yoshitaka and Harada, Tatsuya},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={153--168},
  year={2018}
}

@article{shermin2020adversarial,
  title={Adversarial Network with Multiple Classifiers for Open Set Domain Adaptation},
  author={Shermin, Tasfia and Lu, Guojun and Teng, Shyh Wei and Murshed, Manzur and Sohel, Ferdous},
  journal={IEEE Transactions on Multimedia},
  year={2020},
  publisher={IEEE}
}


% @inproceedings{zhu2019learning,
%   title={Learning feature-to-feature translator by alternating back-propagation for generative zero-shot learning},
%   author={Zhu, Yizhe and Xie, Jianwen and Liu, Bingchen and Elgammal, Ahmed},
%   booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
%   pages={9844--9854},
%   year={2019}
% }

@inproceedings{zhu2019learning,
  title={Learning feature-to-feature translator by alternating back-propagation for generative zero-shot learning},
  author={Zhu, Yizhe and Xie, Jianwen and Liu, Bingchen and Elgammal, Ahmed},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9844--9854},
  year={2019}
}

@inproceedings{schonfeld2019generalized,
  title={Generalized zero-and few-shot learning via aligned variational autoencoders},
  author={Schonfeld, Edgar and Ebrahimi, Sayna and Sinha, Samarth and Darrell, Trevor and Akata, Zeynep},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={8247--8255},
  year={2019}
}

@inproceedings{schonfeld2019generalized,
  title={Generalized zero-and few-shot learning via aligned variational autoencoders},
  author={Schonfeld, Edgar and Ebrahimi, Sayna and Sinha, Samarth and Darrell, Trevor and Akata, Zeynep},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={8247--8255},
  year={2019}
}

% @inproceedings{Huang_2019_CVPR,
%   title={Generative dual adversarial network for generalized zero-shot learning},
%   author={Huang, He and Wang, Changhu and Yu, Philip S and Wang, Chang-Dong},
%   booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
%   pages={801--810},
%   year={2019}
% }


@inproceedings{Huang_2019_CVPR,
  title={Generative dual adversarial network for generalized zero-shot learning},
  author={Huang, He and Wang, Changhu and Yu, Philip S and Wang, Chang-Dong},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={801--810},
  year={2019}
}

@inproceedings {Li19Leveraging, 	
 title = {Leveraging the Invariant Side of Generative Zero-Shot Learning}, 	
 booktitle = {IEEE Computer Vision and Pattern Recognition (CVPR)}, 	
 year = {2019}, 	
 author = {Li, Jingjing and Jing, Mengmeng and Lu, Ke and Ding, Zhengming and Zhu, Lei and Huang, Zi}
} 

% @inproceedings{narayan2020latent,
% 	title={Latent Embedding Feedback and Discriminative Features for Zero-Shot Classification},
% 	author={Narayan, Sanath and Gupta, Akshita and Khan, Fahad Shahbaz and Snoek, Cees GM and Shao, Ling},
% 	booktitle={ECCV},
% 	year={2020}
% }

@inproceedings{narayan2020latent,
	title={Latent Embedding Feedback and Discriminative Features for Zero-Shot Classification},
	author={Narayan, Sanath and Gupta, Akshita and Khan, Fahad Shahbaz and Snoek, Cees GM and Shao, Ling},
	booktitle={ECCV},
	year={2020}
}

@article{narayan2020latent,
  title={Latent embedding feedback and discriminative features for zero-shot classification},
  author={Narayan, Sanath and Gupta, Akshita and Khan, Fahad Shahbaz and Snoek, Cees GM and Shao, Ling},
  journal={arXiv preprint arXiv:2003.07833},
  year={2020}
}

% @article{akata2015label,
%   title={Label-embedding for image classification},
%   author={Akata, Zeynep and Perronnin, Florent and Harchaoui, Zaid and Schmid, Cordelia},
%   journal={IEEE transactions on pattern analysis and machine intelligence},
%   volume={38},
%   number={7},
%   pages={1425--1438},
%   year={2015},
%   publisher={IEEE}
% }

@article{akata2015label,
  title={Label-embedding for image classification},
  author={Akata, Zeynep and Perronnin, Florent and Harchaoui, Zaid and Schmid, Cordelia},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={38},
  number={7},
  pages={1425--1438},
  year={2015},
  publisher={IEEE}
}


@inproceedings{chao2016empirical,
  title={An empirical study and analysis of generalized zero-shot learning for object recognition in the wild},
  author={Chao, Wei-Lun and Changpinyo, Soravit and Gong, Boqing and Sha, Fei},
  booktitle={European conference on computer vision},
  pages={52--68},
  year={2016},
  organization={Springer}
}

@inproceedings{lampert2009learning,
  title={Learning to detect unseen object classes by between-class attribute transfer},
  author={Lampert, Christoph H and Nickisch, Hannes and Harmeling, Stefan},
  booktitle={2009 IEEE Conference on Computer Vision and Pattern Recognition},
  pages={951--958},
  year={2009},
  organization={IEEE}
}

@article{lampert2013attribute,
  title={Attribute-based classification for zero-shot visual object categorization},
  author={Lampert, Christoph H and Nickisch, Hannes and Harmeling, Stefan},
  journal={IEEE transactions on pattern analysis and machine intelligence},
  volume={36},
  number={3},
  pages={453--465},
  year={2013},
  publisher={IEEE}
}

@inproceedings{wang2018zero,
  title={Zero-shot learning via class-conditioned deep generative models},
  author={Wang, Wenlin and Pu, Yunchen and Verma, Vinay and Fan, Kai and Zhang, Yizhe and Chen, Changyou and Rai, Piyush and Carin, Lawrence},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={32},
  year={2018}
}
@inproceedings{wen2016discriminative,
  title={A discriminative feature learning approach for deep face recognition},
  author={Wen, Yandong and Zhang, Kaipeng and Li, Zhifeng and Qiao, Yu},
  booktitle={European conference on computer vision},
  pages={499--515},
  year={2016},
  organization={Springer}
}

@inproceedings{zhu2018generative,
  title={A generative adversarial approach for zero-shot learning from noisy texts},
  author={Zhu, Yizhe and Elhoseiny, Mohamed and Liu, Bingchen and Peng, Xi and Elgammal, Ahmed},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={1004--1013},
  year={2018}
}

@inproceedings{felix2018multi,
  title={Multi-modal cycle-consistent generalized zero-shot learning},
  author={Felix, Rafael and Reid, Ian and Carneiro, Gustavo and others},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={21--37},
  year={2018}
}

@inproceedings{verma2018generalized
  title={Generalized zero-shot learning via synthesized examples},
  author={Verma, Vinay Kumar and Arora, Gundeep and Mishra, Ashish and Rai, Piyush},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4281--4289},
  year={2018}
}



@inproceedings{wang2020classes,
  title={Classes Matter: A Fine-grained Adversarial Approach to Cross-domain Semantic Segmentation},
  author={Wang, Haoran and Shen, Tong and Zhang, Wei and Duan, Ling-Yu and Mei, Tao},
  booktitle={European Conference on Computer Vision},
  pages={642--659},
  year={2020},
  organization={Springer}
}

@inproceedings{cui2020gradually,
  title={Gradually vanishing bridge for adversarial domain adaptation},
  author={Cui, Shuhao and Wang, Shuhui and Zhuo, Junbao and Su, Chi and Huang, Qingming and Tian, Qi},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={12455--12464},
  year={2020}
}

@inproceedings{jiang2020implicit,
  title={Implicit class-conditioned domain alignment for unsupervised domain adaptation},
  author={Jiang, Xiang and Lao, Qicheng and Matwin, Stan and Havaei, Mohammad},
  booktitle={International Conference on Machine Learning},
  pages={4816--4827},
  year={2020},
  organization={PMLR}
}

@inproceedings{chen2020adversarial,
  title={Adversarial-learned loss for domain adaptation},
  author={Chen, Minghao and Zhao, Shuai and Liu, Haifeng and Cai, Deng},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  pages={3521--3528},
  year={2020}
}

@inproceedings{tang2020discriminative,
  title={Discriminative adversarial domain adaptation},
  author={Tang, Hui and Jia, Kui},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={34},
  pages={5940--5947},
  year={2020}
}

@inproceedings{zhang2020label,
  title={Label propagation with augmented anchors: A simple semi-supervised learning baseline for unsupervised domain adaptation},
  author={Zhang, Yabin and Deng, Bin and Jia, Kui and Zhang, Lei},
  booktitle={European Conference on Computer Vision},
  pages={781--797},
  year={2020},
  organization={Springer}
}

@inproceedings{tang2020unsupervised,
  title={Unsupervised domain adaptation via structurally regularized deep clustering},
  author={Tang, Hui and Chen, Ke and Jia, Kui},
  booktitle={Proceedings of the IEEE/CVF conference on computer vision and pattern recognition},
  pages={8725--8735},
  year={2020}
}

@inproceedings{bucci2020effectiveness,
  title={On the Effectiveness of Image Rotation for Open Set Domain Adaptation},
  author={Bucci, Silvia and Loghmani, Mohammad Reza and Tommasi, Tatiana},
  booktitle={European Conference on Computer Vision},
  pages={422--438},
  year={2020},
  organization={Springer}
}

@inproceedings{rakshit2020multi,
  title={Multi-source Open-Set Deep Adversarial Domain Adaptation},
  author={Rakshit, Sayan and Tamboli, Dipesh and Meshram, Pragati Shuddhodhan and Banerjee, Biplab and Roig, Gemma and Chaudhuri, Subhasis},
  booktitle={European Conference on Computer Vision},
  pages={735--750},
  year={2020},
  organization={Springer}
}

@inproceedings{luo2020progressive,
  title={Progressive graph learning for open-set domain adaptation},
  author={Luo, Yadan and Wang, Zijian and Huang, Zi and Baktashmotlagh, Mahsa},
  booktitle={International Conference on Machine Learning},
  pages={6468--6478},
  year={2020},
  organization={PMLR}
}



@inproceedings{tan2019weakly,
  title={Weakly supervised open-set domain adaptation by dual-domain collaboration},
  author={Tan, Shuhan and Jiao, Jiening and Zheng, Wei-Shi},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition},
  pages={5394--5403},
  year={2019}
}

@inproceedings{baktashmotlagh2019learning,
  title={Learning factorized representations for open-set domain adaptation},
  author={Baktashmotlagh, Mahsa and Faraki, Masoud and Drummond, Tom and Salzmann, Mathieu},
  booktitle={7th International Conference on Learning Representations, ICLR 2019},
  year={2019},
  organization={International Conference on Learning Representations, ICLR}
}

@inproceedings{vyas2020leveraging,
  title={Leveraging seen and unseen semantic relationships for generative zero-shot learning},
  author={Vyas, Maunil R and Venkateswara, Hemanth and Panchanathan, Sethuraman},
  booktitle={European Conference on Computer Vision},
  pages={70--86},
  year={2020},
  organization={Springer}
}

@inproceedings{chen2020boundary,
  title={A Boundary Based Out-of-Distribution Classifier for Generalized Zero-Shot Learning},
  author={Chen, Xingyu and Lan, Xuguang and Sun, Fuchun and Zheng, Nanning},
  booktitle={European Conference on Computer Vision},
  pages={572--588},
  year={2020},
  organization={Springer}
}

@inproceedings{xie2020region,
  title={Region graph embedding network for zero-shot learning},
  author={Xie, Guo-Sen and Liu, Li and Zhu, Fan and Zhao, Fang and Zhang, Zheng and Yao, Yazhou and Qin, Jie and Shao, Ling},
  booktitle={European Conference on Computer Vision},
  pages={562--580},
  year={2020},
  organization={Springer}
}

@inproceedings{wan2019transductive,
  title={Transductive Zero-Shot Learning with Visual Structure Constraint},
  author={Wan, Ziyu and Chen, Dongdong and Li, Yan and Yan, Xingguang and Zhang, Junge and Yu, Yizhou and Liao, Jing},
  booktitle={33rd Conference on Neural Information Processing Systems (NeurIPS 2019)},
  year={2019}
}

@article{yu2019zero,
  title={Zero-shot Learning via Simultaneous Generating and Learning},
  author={Yu, Hyeonwoo and Lee, Beomhee},
  journal={Advances in Neural Information Processing Systems},
  volume={32},
  pages={46--56},
  year={2019}
}

@inproceedings{elhoseiny2019creativity,
  title={Creativity inspired zero-shot learning},
  author={Elhoseiny, Mohamed and Elfeki, Mohamed},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={5784--5793},
  year={2019}
}

@inproceedings{liu2019attribute,
  title={Attribute attention for semantic disambiguation in zero-shot learning},
  author={Liu, Yang and Guo, Jishun and Cai, Deng and He, Xiaofei},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={6698--6707},
  year={2019}
}

@inproceedings{jiang2019transferable,
  title={Transferable contrastive network for generalized zero-shot learning},
  author={Jiang, Huajie and Wang, Ruiping and Shan, Shiguang and Chen, Xilin},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision},
  pages={9765--9774},
  year={2019}
}

@inproceedings{arjovsky2017wasserstein,
  title={Wasserstein generative adversarial networks},
  author={Arjovsky, Martin and Chintala, Soumith and Bottou, L{\'e}on},
  booktitle={International conference on machine learning},
  pages={214--223},
  year={2017},
  organization={PMLR}
}

@article{kingma2013auto,
  title={Auto-encoding variational bayes},
  author={Kingma, Diederik P and Welling, Max},
  journal={arXiv preprint arXiv:1312.6114},
  year={2013}
}
